Do the Test Smells Assertion Roulette and Eager Test Impact Students' Troubleshooting and Debugging Capabilities?

To ensure the quality of a software system, developers perform an activity known as unit testing, where they write code (known as test cases) that verifies the individual software units that make up the system. Like production code, test cases are subject to bad programming practices, known as test smells, that hurt maintenance activities. An essential part of most maintenance activities is program comprehension which involves developers reading the code to understand its behavior to fix issues or update features. In this study, we conduct a controlled experiment with 96 undergraduate computer science students to investigate the impact of two common types of test smells, namely Assertion Roulette and Eager Test, on a student's ability to debug and troubleshoot test case failures. Our findings show that students take longer to correct errors in production code when smells are present in their associated test cases, especially Assertion Roulette. We envision our findings supporting academia in better equipping students with the knowledge and resources in writing and maintaining high-quality test cases. Our experimental materials are available online: https://wajdialjedaani.github.io/testsmellstd/

==> Charts/Survey_Q2.tex <==
% \begin{figure*}[ht!]
%      \centering
% \caption*{The process of finding the errors detected by the test cases
% was smooth and easy?}

%      \begin{tabular}{W{c}{0.25\textwidth}W{c}{0.25\textwidth}W{c}{0.25\textwidth}}
% % \begin{subfigure}[b]{0.53\linewidth}
% %  \begin{tikzpicture}[scale=0.80,line join=round, font=\small]
% % %   \pie[radius= 1.6, rotate=180, text=inside] {43.62/Documentations, 13.72/Videos, 42.66/Live streaming} 
% %   {0/Strongly disagree,
% %   10.4/Disagree, 14.6/Neutral, 37.5/Agree, 37.5/Strongly Agree}

% %  \end{tikzpicture}
% % %  \caption{Non-Test Smell}
% % \end{subfigure}
% % &
% \begin{subfigure}[b]{0.15\linewidth}
%  \begin{tikzpicture}[scale=0.80,line join=round, font=\small]
%   \pie[radius= 1.6, rotate=180, text=inside]   {0/Strongly disagree,
%   10.4/Disagree, 14.6/Neutral, 37.5/Agree, 37.5/Strongly Agree}
%  \end{tikzpicture}
% %   \caption{Assertion Roulette}
% \end{subfigure}
% &
% \begin{subfigure}[b]{0.53\linewidth}
%  \begin{tikzpicture}[scale=0.80,line join=round, font=\small]
%   \pie[radius= 1.6, rotate=180, text=inside]   {0/Strongly disagree,
%   10.4/Disagree, 14.6/Neutral, 37.5/Agree, 37.5/Strongly Agree}
%  \end{tikzpicture}
% %   \caption{Assertion Roulette}
% \end{subfigure}
% &
% \begin{subfigure}[b]{0.53\linewidth}
%  \begin{tikzpicture}[scale=0.80,line join=round, font=\small]
%   \pie[radius= 1.6, rotate=180, text=inside]   {0/Strongly disagree,
%   10.4/Disagree, 14.6/Neutral, 37.5/Agree, 37.5/Strongly Agree}
%  \end{tikzpicture}
% %   \caption{Eager Test}
% \end{subfigure}
% \\ 
% \textbf{(A) Non-Test Smell} & \textbf{(B) Assertion Roulette}   & \textbf{(C) Eager Test}\\
% \end{tabular}
%   \vspace{-0.4cm}
%  \caption{Learning material \wajdi{Edit}.}
% \vspace{-0.4cm}
% \label{fig:Learning_Issues}
% \end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[h]
\centering
\caption*{The process of finding the errors detected by the test cases was smooth and easy?}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccc}

\begin{tikzpicture}
\begin{scope}[scale=0.55]
% Pie chart 1
\pie[text=pin]
{3/Strongly disagree, 0/Disagree, 14/Neutral, 28/Agree, 55/Strongly Agree}
 \end{scope}
\end{tikzpicture}
% Pie chart Non-Test Smell
&
\begin{tikzpicture}
\begin{scope}[scale=0.55]
\pie[
    %pos = {8,0},
    % rotate = 120,
    text=pin]
{6/Strongly disagree, 9/Disagree, 18/Neutral, 27/Agree, 40/Strongly Agree}
 \end{scope}
\end{tikzpicture}
% Pie chart Assertion Roulette
&
\begin{tikzpicture}
\begin{scope}[scale=0.55]
 \pie[
    pos = {16,0},
    rotate = 160,
    text=pin]
{0/Strongly disagree, 3/Disagree, 15/Neutral, 32/Agree, 50/Strongly Agree}
 \end{scope}
\end{tikzpicture}
\\% &
\textbf{(A) Non-Test Smell} & \textbf{(B) Assertion Roulette}   & \textbf{(C) Eager Test}\\


\end{tabular}}

 \caption{Percentage of \wajdi{Edit}.}
\label{fig:sentimentAnalyzerVoting}
\end{figure*}




==> Charts/Survey_Q3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\centering
\caption*{Did you find the structure of the test cases easy for you to point out where the error is located?}

\begin{tikzpicture}
\begin{scope}[scale=0.5]
\pie[text=pin]
{0/Strongly disagree,
10.4/Disagree,
14.6/Neutral,
37.5/Agree,
37.5/Strongly Agree}
\end{scope}
\end{tikzpicture}
\caption{Caption here \wajdi{break this by group}}
\label{DataSource}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
